Admissible function spaces for weighted Sobolev inequalities

Let $k,N \in \mathbb{N}$ with $1\le k\le N$ and let $\Omega=\Omega_1 \times \Omega_2$ be an open set in $\mathbb{R}^k \times \mathbb{R}^{N-k}$. For $p\in (1,\infty)$ and $q \in (0,\infty),$ we consider the following Hardy-Sobolev type inequality: \begin{align} \int_{\Omega} |g_1(y)g_2(z)| |u(y,z)|^q \, dy \, dz \leq C \left( \int_{\Omega} | \nabla u(y,z) |^p \, dy \, dz \right)^{\frac{q}{p}}, \quad \forall \, u \in \mathcal{C}^1_c(\Omega), \end{align} for some $C>0$. Depending on the values of $N,k,p,q,$ we have identified various pairs of Lorentz spaces, Lorentz-Zygmund spaces and weighted Lebesgue spaces for $(g_1, g_2)$ so that the above inequality holds. Furthermore, we give a sufficient condition on $g_1,g_2$ so that the best constant in the above inequality is attained in the Beppo-Levi space $\mathcal{D}^{1,p}_0(\Omega)$-the completion of $\mathcal{C}^1_c(\Omega)$ with respect to $\|\nabla u\|_{L^p(\Omega)}$.

==> new.tex <==
In the following, we give definition of Morrey space introduced by Morrey in \cite{Morrey}.
\begin{definition}[Morrey's space]\label{def-Morrey}
For $p,q \in (0, \infty]$ with $q \le p$ and $g \in L_{loc}^q(\RN)$ consider the following quantity:
$$\norm{g}_{\M^{p,q}(\RN)} := \sup_{\{x\in \R^N,r>0\}} |B_r(x)|^{\frac{1}{p}-\frac{1}{q}} \left( \int_{B_r(x)}|g(y)|^q \, \dy \right)^{\frac{1}{q}}.$$
Then the Morrey space $\M^{p,q}(\RN)$ is defined as $$\M^{p,q}(\RN):= \left\{g \in L_{loc}^q(\RN): \norm{g}_{\M^{p,q}(\RN)} < \infty \right\}.$$
\end{definition}
\begin{remark}\label{Morrey}
For $q=p$, $\M^{p,p}(\RN)$ coincides with $L^p(\RN)$ and for $q<p$ using Remark \ref{equivalent}, $\M^{p,q}(\RN) \supset L^{p, \infty}(\RN)$.
\end{remark}












@inproceedings {Muckenhoupt1978,
    AUTHOR = {Muckenhoupt, B.},
     TITLE = {Weighted norm inequalities for classical operators},
 BOOKTITLE = {Harmonic analysis in {E}uclidean spaces ({P}roc. {S}ympos.
              {P}ure {M}ath., {W}illiams {C}oll., {W}illiamstown, {M}ass.,
              1978), {P}art 1},
    SERIES = {Proc. Sympos. Pure Math., XXXV, Part},
     PAGES = {69--83},
 PUBLISHER = {Amer. Math. Soc., Providence, R.I.},
      YEAR = {1979},
   MRCLASS = {42B25 (42B20 42B30)},
  MRNUMBER = {545240},
MRREVIEWER = {Alberto Torchinsky},
}


@article {Farman,
    AUTHOR = {Mamedov, Farman and Shukurov, Yashar},
     TITLE = {A {S}awyer-type sufficient condition for the weighted
              {P}oincar\'{e} inequality},
   JOURNAL = {Positivity},
  FJOURNAL = {Positivity. An International Mathematics Journal Devoted to
              Theory and Applications of Positivity},
    VOLUME = {22},
      YEAR = {2018},
    NUMBER = {3},
     PAGES = {687--699},
      ISSN = {1385-1292},
   MRCLASS = {35A23 (26D10 35J15 35J70)},
  MRNUMBER = {3817112},
       DOI = {10.1007/s11117-017-0537-2},
       URL = {https://doi.org/10.1007/s11117-017-0537-2},
}
\noi $(ii)$ \tb{ For $N>p$ and $q\in[p,p^*]$, we have shown that $L^{\al(p,q), \infty}(\RN) \subset \pqR$ (see Theorem \ref{Symmetrization}). Here we give an alternate proof of this result by showing that every weight function in $L^{\al(p,q), \infty}(\RN)$ satisfies \eqref{SW}. Let $g \in L^{\al(p,q), \infty}(\RN)$. For any $r>1$, using $(i)$ of Proposition \ref{Lorentz properties} we get $|g|^r \in L^{\frac{\al(p,q)}{r}, \infty}(\RN)$. Thus
\begin{align}\label{re-ineq}
   \sup_{t>0} t^{\frac{r}{\al(p,q)}-1} \int_{0}^t (|g|^r)^*(t) \, \dt \le C.
\end{align}
Now 
\begin{align*}
    \sup_{t>0} t^{\frac{r}{\al(p,q)}-1} \int_{0}^t (|g|^r)^*(t) \, \dt & = \left( \sup_{t>0} t^{\frac{1}{\al(p,q)} - \frac{1}{r}} \left( \int_{0}^t (|g|^r)^*(t) \, \dt \right)^{\frac{1}{r}} \right)^r \\
    & = \left( \sup_{l>0} l^{N \left( \frac{1}{\al(p,q)} - \frac{1}{r} \right)} \left( \int_{0}^{l^N} (|g|^r)^*(t) \, \dt \right)^{\frac{1}{r}} \right)^r,
\end{align*}
where $|Q|=l^N$. Therefore, from \eqref{re-ineq} and the Hardy-Littlewood inequality (Proposition \ref{HL and PS}), we get 
\begin{align*}
   \sup_{Q \subset \RN, |Q| < \infty} |Q|^{\frac{1}{\al(p,q)} - \frac{1}{r}} \left( \int_{Q} |g(x)|^r \, \dx \right)^{\frac{1}{r}} \le C.
\end{align*}
Thus $g$ satisfies \eqref{SW} and hence $g \in \pqR$. }


$(i)$ \tr{ Let $g \in L_{loc}^1(\RN)$ and $g$ satisfies the following weighted inequality for fractional integral:
 \begin{align}\label{fractional}
     \intRn |g(x)| \left[ I(f)(x) \right]^q  \, \dx  \le C \left( \intRn f(x)^p \, \dx \right)^{\frac{q}{p}}, \quad \forall \, f \ge 0,
 \end{align}
 where $I(f)(x) := \int_{\RN} \frac{|f(y)|}{|x-y|^{N-1}} \, \dy$. We will show that $g \in \pqR.$  Let $u \in \c1(\RN)$. Using (1.2) of \cite{Sawyer} we have
 \begin{align*}
     |u(x)| \le C I(|\nabla u|)(x)  \; \text{ in }  \R^N, 
 \end{align*}
where $C = C(N)>0$. By taking $f = |\Gr u|$ in \eqref{fractional} and using the above inequality, we get 
 \begin{align*}
     \intRn |g(x)| |u(x)|^q \, \dx \le C \left( \intRn |\Gr u(x)|^p \, \dx \right)^{\frac{q}{p}}, \quad \forall \, u \in \c1(\RN).
 \end{align*}
 Thus $g \in \pqR$. }
 
 %\noi \cite{M1972},1972: Muckenhoupt gave sufficient condition for (p,p) with $g=h$.

%\noi \cite{MW1974}, 1974: Muckenhoupt and Wheeden gave sufficient condition for (p,q) with $g=h$.

%\noi \cite{Chan_Whed}, 1985: \tr{Got the citation for (p,p). Check Theorem 1.2 and 1.3 of the paper Chanillo-Wheeden in Dropbox.}  

%\noi \cite{Muckenhoupt1978}: Muckenhoupt raised the general question of characterizing functions when the weighted norm inequality \eqref{Weighted-Riesz} holds.


%\noi \cite{Karman-Sawyer},1985: Karman and Sawyer. This is the paper which talks about Fefferman's result and convolution type inequality. They have given a sufficient condition for the convolution type inequality.

%\noi \cite{LN},1988: Long and Nie have given a sufficient condition (an integral condition involving $I$) on $g,h$ so that \eqref{two_weight_ineq} holds, see \cite[Theorem 2.1, Corollary 2.1]{LN}. \tb{They have actually given the sufficient condition for \eqref{two_weight_ineq} directly, not for the convolution inequality.} 

%\noi \cite{Perez},1990: In this paper, Corollary 1.6 concerns weights of the form $(g,1)$. They have given a necessary and sufficient condition on $g \in A_{\infty}$ so that \eqref{two_weight_ineq} holds.

%\noi \cite{Sawyer},1992: Sawyer gives a necessary and also a sufficient condition for the convolution type inequality in Theorem 1. In Theorem 5, he considers \eqref{two_weight_ineq} on cubes and given a sufficient condition.

 

==> p.tex <==
\parskip.25cm
\usepackage{amsmath,amssymb,amsthm,amsfonts,epsfig,enumerate}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{mathrsfs,amssymb,soul}
\usepackage[utf8]{inputenc}
\usepackage{amsmath,amssymb,amsthm,amsfonts,epsfig,enumerate}
\usepackage{pst-plot,pst-node}
\usepackage{xfrac}




\renewcommand{\baselinestretch}{1}
\allowdisplaybreaks[4] 

\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=myblue,
    filecolor=magenta,      
    urlcolor=mygreen,
    citecolor=mygreen,
}
\definecolor{mygreen}{rgb}{0.01,0.6,0.2}
\definecolor{myblue}{rgb}{0.01, 0.18, 1.0}
\textwidth6.25in \textheight9in \hoffset-0.5in \voffset-0.5in



\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{Lemma}[definition]{Lemma}
\newtheorem{result}[definition]{Result}
\theoremstyle{definition}
\newtheorem{remark}[definition]{Remark}
\newtheorem{example}[definition]{Example}
\numberwithin{equation}{section}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\norm{\lVert}{\rVert}%
\makeatletter
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\newcommand{\al} {\alpha}
\newcommand{\aln} {\alpha_n}
\newcommand{\pa} {\partial}
\newcommand{\be} {\beta}
\newcommand{\de} {\delta}
\newcommand{\De} {\Delta}
\newcommand{\Dep} {\Delta_p}
\newcommand{\ga} {\gamma}
\newcommand{\Ga} {\Gamma}
\newcommand{\om} {\omega}
\newcommand{\Om} {\Omega}
\newcommand{\en} {\eta^n}
\newcommand{\ei} {\eta^i}
\newcommand{\la} {\lambda}
\newcommand{\La} {\Lambda}
\newcommand{\si} {\sigma}
\newcommand{\Si} {\Sigma}
\newcommand{\Gr} {\nabla}
\newcommand{\no} {\nonumber}
\newcommand{\noi} {\noindent}
\newcommand{\vph} {\varphi}
\newcommand{\eps} {\varepsilon}
\newcommand{\ep} {\epsilon}
\newcommand{\ra} {\rightarrow}
\newcommand{\embd} {\hookrightarrow}
\newcommand{\wra} {\rightharpoonup}
\newcommand{\intRn}{\displaystyle{\int_{\mathbb{R}^N}}}
\newcommand{\Int}{{\displaystyle \int}}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  
  
\left.\kern-\nulldelimiterspace % automatically resize the bar with \right
#1 % the function
% \vphantom{\big|} % pretend it's a little taller at normal size
\right|_{#2} % this is the delimiter
}}
\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\br}[1]{\autobracket*{#1}}
\DeclarePairedDelimiter\autoset{\{}{\}}
\newcommand{\set}[1]{\autoset*{#1}}
\def\inpr#1{\left\langle #1\right\rangle}
\renewcommand\baselinestretch{1.1}
\def\vol{\mathrm{vol}}
\def\B{{\widetilde B}}
\def\w{{\widetilde w}}
\def\t{\tau}
\def \tb {\textcolor{blue}}
\def \tr {\textcolor{red}}

\def\wp{{W^{1,p}(\Om)}}
\def\wRN{{W^{1,p}(\RN)}}
\def\wN{{W^{1,N}(\Om)}}
\def\Bf{\mathbf}
\def\A{{\mathcal A}}
\def\B{{\mathcal B}}
\def\C{{\mathcal C}}
\def\D{{\mathcal D}}
\def\E{{\mathcal E}}
\def\J{{\mathcal J}}
\def\K{{\mathcal K}}
\def\P{{\Phi}}
\def\M{{\mathcal M}}
\def\S{{\mathcal S}}
\def\T{{\mathcal T}}
\def\U{{\mathcal U}}
\def\O{{\mathcal O}}
\def\mR{{\mathcal R}}
\def\hs{\hspace}
\def\R{{\mathbb R}}
\def\Rc{{\mathcal R}}
\def\RN{{\mathbb R}^N}
\def\N{{\mathbb N}}
\def\F{{\mathcal F}}
\def\G{{\mathcal G}}
\def\({{\Big(}}
\def\){{\Big)}}
\def\wsd{{\F_d}}
\def\wsp{{\F_{\frac{N}{p}}}}
\def\c{{\C^1}}
\def\dis{{\displaystyle \int_{\Omega}}}
\def\disb{{\displaystyle \int_{B^c_1}}}
\def\tphi{{\tilde{\phi}}}
\def\resb{{C_c^1(\overline{B_1^c})}}
\def\p{{p^{\prime}}}
\def\r{{r^{\prime}}}
\def\Np{{N^{\prime}}}
\def\g{{\tilde{g}}}
\def\dr{{\rm d}r}
\def\dS{{\rm d}S}
\def\ds{{\rm d}s}
\def\dS{{\rm d}S}
\def\dt{{\rm d}t}
\def\dx{{\rm d}x}
\def\dy{{\rm d}y}
\def\dxp{{\rm d}x^{\prime}}
\def\dJ{{\rm d}J}
\def\dJl{{\rm d}(J - \lambda G)}
\def\dsg{{\rm d}\sigma}
\def\pa{{\partial}}
\def\dispa{{\displaystyle \int_{\partial \Omega}}}
\def\hm{{\mathcal{H}}^{N-1}}
\def\pcr{{\frac{p(N-1)}{N-p}}}
\def\Phl{{\Phi_{\lambda}}}
\def\tphi{{\tilde{\phi}}}
\def\tPhi{{\tilde{\Phi}}}
\def\Lp{{L^{(\alpha + 1)p}}}
\def\Lpr{{L^{(\alpha + 1)p r^{\prime}}}}
\def\xp{{x^{\prime}}}
\usepackage[hyperpageref]{backref}
\def\lfrac#1#2{{\scriptstyle\frac{#1}{#2}}}
\def\llfrac#1#2{{\scriptscriptstyle\frac{#1}{#2}}}
\DeclareMathOperator*\lowlim{\underline{lim}}
\DeclareMathOperator*\uplim{\overline{lim}}
\newcommand{\pq}{\mathcal{H}_{p,q}(\Om)}
\newcommand{\pqo}{\mathcal{H}_{p,q_1}(\Om)}
\newcommand{\pqt}{\mathcal{H}_{p,q_2}(\Om)}
\newcommand{\tq}{\mathcal{H}_{2,q}(\Om)}
\newcommand{\pp}{\mathcal{H}_{p,p}(\Om)}
\newcommand{\two}{\mathcal{H}_{2,2}}
\newcommand{\pqR}{\mathcal{H}_{p,q}(\mathbb{R}^N)}
\newcommand{\pqab}{\mathcal{H}^{p,q}(\Om_{a,b,S})}
\newcommand{\dpp}{\D_0^{1,p}}
\newcommand{\Dp}{\D_0^{1,p}(\Om)}
\newcommand{\DN}{\D_0^{1,N}(\Om)}
\newcommand{\Dtwo}{\D_0^{1,2}(\Om)}
\newcommand{\intRn}{\displaystyle{\int_{\mathbb{R}^N}}}
\newcommand{\intRnn}{\displaystyle{\int_{\mathbb{R}^{N-1}}}}
\newcommand{\intRnu}{\displaystyle{\int_{\mathbb{R}^N_{+}}}}
\newcommand{\intRk}{\displaystyle{\int_{\mathbb{R}^k}}}
\newcommand{\intRnk}{\displaystyle{\int_{\mathbb{R}^{N-k}}}}
\newcommand{\wrastar} {\overset{\ast}{\rightharpoonup}}
\newcommand{\intRno}{\displaystyle{\int_{\mathbb{R}^{N-1}}}}
\newcommand{\intRnone}{\displaystyle{\int_{\mathbb{R}^{N-1}}}}
\newcommand{\intRz}{\displaystyle{\int_{\mathbb{R}^{N}_{z}}}}
\newcommand{\intRx}{\displaystyle{\int_{\mathbb{R}^{N}_{x^{\prime}}}}}
\newcommand{\Bc}{B^c_1}
\newcommand{\intBc}{\displaystyle{\int_{B_1^c}}}
\newcommand{\Int}{{\displaystyle \int}}
%\newcommand{\Int}[1]{\displaystyle{\int_{#1}}}
\newcommand{\intom}{\displaystyle{\int_{|\om|=1}}}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
 % \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}
  
\renewcommand\baselinestretch{1.1}
\usepackage[hyperpageref]{backref}


\NewDocumentCommand{\intervals}{ m m }{#1 {,} #2}




\def\vol{\mathrm{vol}}
\def\B{{\widetilde B}}
\def\w{{\widetilde w}}
\def\t{\tau}
\def \tb {\textcolor{blue}}
\def \tr {\textcolor{red}}
\def \tg {\textcolor{green}}

\def\inpr#1{\left\langle #1\right\rangle}
\def\wp{{W^{1,p}_0(\Om)}}
\def\wRN{{W^{1,p}(\RN)}}
\def\dpR{{\D^{1,p}_0(\RN)}}
\def\dpo{{\D^{1,p}_0(\Omega_1 \times \Omega_2)}}
\def\wpb{{W^{1,p}(B_1^c)}}
\def\wNb{{W^{1,N}(B_1^c)}}
\def\wN{{W^{1,N}_0(\Om)}}
\def\wpl{{{ W}^{1,p}_{loc}(\Om)}}
\def\Bf{\mathbf}
\def\A{{\mathcal A}}
\def\C{{\mathcal C}}
\def\D{{\mathcal D}}
\def\E{{\mathcal E}}
\def\mH{{\mathcal H}}
\def\J{{\mathcal J}}
\def\K{{\mathcal K}}
\def\N{{\mathbb N}}
\def\F{{\mathcal F}}
\def\M{{\mathcal M}}
\def\S{\mathbb{S}}
\def\T{{\mathcal T}}
\def\mR{{\mathcal R}}
\def\hs{\hspace}
\def\cp{{\rm Cap}_p}
\def\cset{{\subset \subset }}
\def\R{{\mathbb R}}
\def\RN{{\mathbb R}^N}
\def\Rk{{\mathbb R}^k}
\def\RNk{{\mathbb R}^{N-k}}
\def\RNz{{\mathbb R}^N_{z}}
\def\Rx{{\mathbb R}^N_{x^{\prime}}}
\def\({{\Big(}}
\def\){{\Big)}}
\def\wsd{{\F_d}}
\def\wsp{{\F_{\frac{N}{p}}}}
\def\ws2{{\F_{\frac{N}{2}}}}
\def\cc{{\C_c^\infty}}
\def\c1{{\C_c^1}}
\def\dis{{\displaystyle \int_{\Omega}}}
\def\disab{{\displaystyle \int_{\Omega_{a,b,S}}}}
\def\disone{{\displaystyle \int_{\Omega_1}}}
\def\distwo{{\displaystyle \int_{\Omega_2}}}
\def\disR{{\displaystyle \int_{\mathbb{R}^N}}}
\def\disC{{\displaystyle \int_{\C}}}
\def\disH{{\displaystyle \int_{\mH}}}
\def\tphi{{\tilde{\phi}}}
\def\psix{{\psi_{\xp}}}
\def\p{{p^{\prime}}}
\def\q{{q^{\prime}}}
\def\r{{r^{\prime}}}
\def\Np{{N^{\prime}}}
\def\f{{\tilde{f}}}
\def\g{{\tilde{g}}}
\def\h{{\tilde{h}}}
\def\d{{\rm d}}
\def\dr{{\rm d}r}
\def\dS{{\rm d}S}
\def\dSk{{{\rm d}S}_k}
\def\dSNk{{{\rm d}S}_{N-k}}
\def\dl{{\rm d}\lambda}
\def\ds{{\rm d}s}
\def\dt{{\rm d}t}
\def\dz{{\rm d}z}
\def\dx{{\rm d}x}
\def\dy{{\rm d}y}
\def\dvr{{\rm d}\varrho}
\def\drho{{\rm d}\rho}
\def\dxp{{\rm d}x^{\prime}}
\def\dxN{{\rm d}x_N}
\def\dJ{{\rm d}J}
\def\xp{{x^{\prime}}}
\def\loc{{L^1_{loc}(B_1^c)}}
\def\locN{{L^N_{loc}(B_1^c)}}
\def\locp{{L^N_{loc}(B_1^c)}}
\def\gz{{\tilde{g}_{z}}}
\def\vpp{{\vph^{\prime}}}
\def\G{{\tilde{G}}}
\def\H{{\mathcal{H}}}
\def\h{{\tilde{h}}}
\def\hg{{\hat{g}_{z}}}
